LQG Control and Sensing Co-Design

We investigate a Linear-Quadratic-Gaussian (LQG) control and sensing co-design problem, where one jointly designs sensing and control policies. We focus on the realistic case where the sensing design is selected among a finite set of available sensors, where each sensor is associated with a different cost (e.g., power consumption). We consider two dual problem instances: sensing-constrained LQG control, where one maximizes control performance subject to a sensor cost budget, and minimum-sensing LQG control, where one minimizes sensor cost subject to performance constraints. We prove no polynomial time algorithm guarantees across all problem instances a constant approximation factor from the optimal. Nonetheless, we present the first polynomial time algorithms with per-instance suboptimality guarantees. To this end, we leverage a separation principle, that partially decouples the design of sensing and control. Then, we frame LQG co-design as the optimization of approximately supermodular set functions; we develop novel algorithms to solve the problems; and we prove original results on the performance of the algorithms, and establish connections between their suboptimality and control-theoretic quantities. We conclude the paper by discussing two applications, namely, sensing-constrained formation control and resource-constrained robot navigation.

==> tex/Introduction_old.tex <==
%!TEX root = ../main.tex

\section{Introduction}\label{sec:Intro}

%% MOTIVATION AND NOVELTY
Traditional approaches to control \edited{of}{dynamical} systems with partially observable state assume the choice of
sensors %(and the actuators)
 used to observe 
 %(and regulate) 
 the system is given.
The choice of sensors usually results from a preliminary design phase in which an 
expert designer selects a suitable sensor suite that accommodates estimation requirements (e.g., observability, 
desired estimation error) and system constraints (e.g., size, cost).
Modern control applications, from large networked systems to miniaturized robotics systems, 
pose serious limitations to the applicability of this traditional paradigm. 
In large-scale networked systems (e.g., smart grids or robot swarms), in which new nodes are continuously 
added and removed from the network, 
a manual re-design of the sensors becomes cumbersome and expensive, and it is simply not scalable. %, and time-consuming.
In miniaturized robot systems, while the set of onboard sensors is fixed, 
it may be desirable to selectively activate only a subset of the sensors during different phases of operation, %, depending on the mission requirements
 in order to minimize % power constraints. 
 power consumption. 
% For instance, a robot may need to spend more effort in sensing when moving at high-speed among 
% obstacles, while o. 
% We note that in 
%
% Nowadays: 
% many sensors and many actuators:
% focus on minimality: jointly consider control-theoretic quantities (controllability or observability), 
% but also account for power, size, cost constraints.
%
%system design
%robotics with resource constraints
%Also in this case, the need to dynamically adjust the sensing prevents a manual design.
%Both application scenarios are characterized by the fact that, 
% In these application scenarios, one usually has access to a (potentially large) list of potential sensors, 
% but, due to resource constraints (e.g., cost, power),   
% These application scenarios advocate for the design of automated approaches for sensor design.  
% More specifically, while in general one has a (potentially large) set of sensors 
%Both application scenarios are characterized by the fact that, despite the availability 
In both application scenarios,
one usually has access to a (possibly large) list of potential sensors, 
but, due to resource constraints (size, weight, power, cost), can only utilize 
a subset of them. Moreover, the need for online and large-scale sensor selection demands for 
% hence advocating for the development of 
 automated approaches that efficiently select a subset of sensors 
 to maximize system performance.
 %for sensor selection. 
 %the selection of a suitable subset of sensors that  ma
 % sensor selection. 
%it is desirable to only 
% utilize a suitable subset of those 
%and needs to select the subset that maximize 
%that maximize a task-dependent performance metric.
% that allows satisfying desired task-dependent objectives.
% they require the design of suitable algorithms that are able to select 
%
% While the problem of sensor design has been studied
%
% Second, tight constraints and dynamically changing conditions
%
% resource allocation
%
% task-driven sensing

Motivated by these applications,
in this paper we consider the problem of jointly designing control, estimation, and 
\edited{sensor selection}{sensing} for a 
system with partially observable state.

\myParagraph{Related work} \LC{literature review should be expanded}
One body of related work is \emph{control over band-limited communication channels}, which 
investigates the trade-offs between communication constraints (e.g., data rate, quantization, delays)
and control performance (e.g., stability) in networked control systems. 
%control goals, such as stability, mean entry times, and asymptotic state norms, emerge naturally.
 %This set of works considers the case in which the controllers are distributed across a 
Early work  provides results on the impact of quantization~\cite{Elia01tac-limitedInfoControl}, finite data 
rates~\cite{Nair04sicon-rateConstrainedControl,Tatikonda04tac-limitedCommControl}, and separation principles for \LQG design with 
communication constraints~\cite{Borkar97-limitedCommControl}; more recent work focuses on privacy constraints~\cite{LeNy14tac-limitedCommControl}. 
We refer the reader to the surveys~\cite{Nair07ieee-rateConstrainedControl,Hespanha07ieee-networkedControl,Baillieul07ieee-networkedControl} \edited{}{for a comprehensive review}.
%as well as to~\cite{Elia01tac-limitedInfoControl,Nair04sicon-rateConstrainedControl,Tatikonda04tac-limitedCommControl,Borkar97-limitedCommControl}, 
%for specific discussion on .
% how much information is actually needed to get good control performance: Control over a communication channel: surveys:
% adjust data rate to preserve stability
% The data rate constraint introduces quantization into the feedback loop - 
% code length \& 
A~second set of related work is \emph{sensor selection and scheduling}, in which one has to select a (possibly time-varying) 
set of sensors in order to monitor a phenomenon of interest. 
Related literature includes approaches based on randomized sensor selection~\cite{gupta2006stochastic}, dual volume sampling~\cite{avron2013faster,li2017dual},
convex relaxations~\cite{joshi2009sensor,leny2011kalman}, and 
submodularity~\cite{shamaiah2010greedy,jawaid2015submodularity,tzoumas2015sensor}. 
% Gupta~\etal~\cite{gupta2006stochastic} propose a randomized sensor schedule that minimizes the error covariance 
% for a sensor network estimating a noisy process.
% Joshi and Boyd~\cite{joshi2009sensor} use convex relaxations to select a set of sensors to maximize estimation performance.
% % \minedit{Jamali-Rad~\etal~\cite{jamali2015distributed} propose a distributed algorithm for solving
% % the centralized sensor scheduling problem with performance guarantees.}
% % More relevant to our discussion is the use of structural properties of the  metric to be optimized, 
% % to enable formal performance guarantees. 
% %here is to focus on the structural properties of the objective function to make it more amenable to optimization. 
% % As discussed in the sequel, \textit{submodularity} is an important property of set functions that facilitates combinatorial optimization in polynomial time via \textit{greedy} algorithms with suboptimality guarantees \cite{nemhauser1978analysis}. 
% Shamaiah~\etal~\cite{shamaiah2010greedy} prove that, over a single time-step, the $\logdet$ of the error covariance of the Kalman filter 
% is supermodular and monotone non-increasing, enabling the use of greedy algorithms for near-optimal sensor selection. 
% %Additionally, the 
% %work~\cite{shamaiah2010greedy} shows through empirical tests that the greedy heuristic outperforms the more computationally intensive semi-definite relaxation of .
% % over multiple time-steps, which relies on convex relaxations and does not provide performance guarantees. 
% Jawaid and Smith~\cite{jawaid2015submodularity} prove that $\logdet$ of the error covariance of the Kalman filter is 
% \emph{sequence supermodular} and monotone non-increasing under technical assumptions. %restrictive assumptions on the system dynamics and parameters.
% %; thus, limiting the versatility of their results. %At the current state of the art, in the framework of sensor placement and optimal Kalman filtering, 
% Tzoumas~\etal~\cite{tzoumas2015sensor} prove that the $\logdet$ of the error covariance from the Kalman filter is supermodular and monotone non-increasing over a finite observation interval. % and a choice of sensor set.
% %Similar effort has been invested in proving submodularity of other estimation error metrics.
% % Jawaid and Smith~\cite{jawaid2015submodularity} provide a counterexample showing that the $\TR$ of the error covariance is not, in general, a supermodular set function. Other counterexamples are given in~\cite{zhang2015sensor}, in the context of sensor selection. One of our goals here is to find specific classes of systems for which 
% % the $\TR$ of the covariance can be proven to be supermodular.
The third set of related works is \emph{information-constrained (or information-regularized)} \LQG 
control~\cite{Shafieepoorfard13cdc-attentionLQG,tanaka2015sdp}.
%Bounded rationality: recently [22] considered an information-constrained LQG control problem,
%Very recent work focuses on joint sensor and LQG design or the so-called the \emph{information-regularized} LQG [Tanaka1]. 
%Bansal89automatica-codesign
Shafieepoorfard and Raginsky~\cite{Shafieepoorfard13cdc-attentionLQG} 
%consider a rational inattention framework for \LQG control
study rationally inattentive control laws for \LQG control and discuss their effectiveness  in stabilizing the system. 
Tanaka and Mitter~\cite{tanaka2015sdp} consider the co-design of sensing, control, and estimation, and propose to augment the standard \LQG cost 
with an information-theoretic regularizer, and derive an elegant solution based on semidefinite programming.
%The main difference between

%In contrast to the previous papers, 
In this paper
% and~\cite{tanaka2015sdp} is that 
we introduce 
%we propose 
% for the first time
%  in the literature
%  the case where 
the co-design problem of sensing, control, and estimation for the case where the choice of sensors, rather than being arbitrary (see, e.g.,~\cite{tanaka2015sdp}), is restricted to a finite selection from a set of available sensors.
%is restricted by the choice of sensors, which, rather than being arbitrary (see, e.g.,~\cite{tanaka2015sdp}), is restricted to a finite selection from a set of available sensors.
%In~addition, we account for the case where each sensor selection is associated with a (possibly different) cost, which captures, for example, the sensor's different monetary cost, impact to power consumption, or bandwidth utilization. 
%\LC{worth mentioning that we consider heterogeneous costs and we consider the 2 variants of the problem.}
%\VT{Vassilis notes: Mention Jegelka's and Boutsidis works on column selection in such a way that it is clear that their contributions do not apply in the solution of this problem. As I note in the Future Work, it would be really interesting to see how we can construct an algorithm that achieves an approximation bound with respect to the case where all sensors are selected.}

\myParagraph{Contributions}
We introduce  the \emph{\LQG control and sensing co-design} problem, that 
extends Linear-Quadratic-Gaussian (\LQG) control  to the case where, besides 
designing an optimal controller and estimator, one has to select a set of sensors to observe the system state. 
\edited{In our formulation we also account for the case where each sensor is associated with a (possibly different) selection cost, and capture that way the practical scenarios where each sensor may have a different monetary cost, impact to power consumption, or bandwidth utilization.}{In our formulation, each sensor is associated with a \emph{cost} that quantifies the penalty incurred when using that sensor (trivially, if there is no cost associated to using a sensor, one would always prefer to select and use all available sensors). 
We consider the general case in which each sensor has a potentially different cost, 
hence capturing the practical scenarios where each sensor may have a different monetary cost, power consumption, or bandwidth utilization.}% and produce the measurements to be fed to the estimator.
% In this paper, we introduce the \emph{sensing-constrained \LQG control} problem, in which one has 
% to jointly design sensing, estimation, and control, under given constraints on the resources spent for sensing.
%optimal \emph{sensing strategy}, a controller, and an estimator.
%to design an \emph{optimal sensing strategy}, besides computing an optimal controller and estimator.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% CONTRIBUTIONS
% Problem Formulation
% Separation Principle
% Algorithms
% Performance bounds: depending on the submodularity ratio
% - Algorithm 2 is the first scalable algorithm with provable suboptimality guarantees for the minimization of a (possibly) approxi- mately supermodular function
% - Algorithm 4 is the first scalable algorithm with provable suboptimality guarantees for the minimum heterogeneous-cost set-selection subject to a constraint on an approximately supermodular function
% provide a computable lower bound for the submodularity ratio, and establish control-theoretic conditions for the validity of this lower bound.
% - experiments

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Problem Formulation
In more detail, we formulate two dual instances of the {\LQG co-design} problem.
The first instance, named \emph{sensing-constrained \LQG control}, 
involves the joint design of the controller, estimator, and sensing policies 
that minimize the \LQG objective (quantifying tracking performance and control effort) 
while satisfying a given constraint on the \edited{}{maximum admissible} cost of the selected sensors. % sensing policy.
% In practice, the sensing constraint is due to the cost of th 
The second instance, named \emph{minimum-sensing \LQG control},
 involves the joint design of the controller, estimator, and sensing policies 
that minimize the cost of the selected sensors while satisfying a given \edited{}{lower-bound on the} \LQG performance.  
%we account for the case where each sensor selection is associated with a (possibly different) cost.
% In particular, we formulate the \emph{sensing-constrained} (finite-horizon) \LQG  problem as
% the joint design of an optimal control and estimation policy, as well as the
% selection of a subset of $k$ out of $N$ available sensors, that 
%\LC{here it would be nice to have each paragraph describing a contribution of the paper.
% We are making the following contributions: (i) problem formulation (this is the paragraph above), (ii) fast algorithms with provable performance guarantees, 
% (iii) experimental evaluation that shows that the problem is relevant in practical applications and that they have excellent performance.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Separation Principle
% Algorithms


%. %, which quantifies the tracking performance and the control effort. 
While the computation of the optimal sensing strategies is combinatorial in nature,
%can be intractable, being a combinatorial problem,
%\VT{State that the sensing-constrained LQG control problem is NP-hard}
% Contrarily to related work, we focus on the realistic case in which the  sensing strategy 
% has to be selected among a finite set of possible sensing modalities. 
% We show that a separation principle holds, which allows the design of sensing, estimation, and control policies 
% in isolation. 
%a key contribution of this paper is to 
\edited{}{we provide the first scalable algorithms that compute control, estimation, and sensing strategies with provable 
sub-optimality guarantees. Towards this goal, we leverage a separation principle to show that the design of sensing, control, and estimation, can be partially decoupled, and use and develop tools for the optimization of \mbox{(approximately) supermodular set functions.}}  


\edited{In particular, the proposed algorithms enjoy the following two properties: (i)~they are the first scalable algorithms for the optimization of (approximately) supermodular functions subject to heterogeneous-cost set-selection considerations; and (ii)~they can exhibit superior approximation performance guarantees even when used for the optimization of (exactly) supermodular functions.}{More generally, the proposed algorithms (i) are the first scalable algorithms for the optimization of (approximately) supermodular functions subject to heterogeneous-cost constraints, and (ii)~exhibit superior approximation performance guarantees even when used for the optimization of (exactly) supermodular functions.}  For~example, the proposed algorithm for the sensing-constrained \LQG control problem is the first scalable algorithm with provable suboptimality guarantees for the optimization of (approximately) supermodular functions subject to heterogeneous-cost set-selection constraints, and although it has the same running time as its counterparts in the (exactly) supermodular function optimization literature, it can achieve the approximation performance bound $(1-1/e)$, which is superior to the previously established bound $1/2(1-1/e)$ in the literature~\cite{krause2005note} (details on the performance of the proposed algorithms are found in Section~\ref{sec:guarantees}).  
%have the property that if used for the  in addition, the proposed algorithms also guarantee superior approximation performance for the case of exactly supermodular optimization subject to heterogeneous set selection considerations.  }  % the sensing-constrained
%\LC{here you can add a couple of sentences about the technical tools or something more quantitative about the performance guarantees/algorithms.}
%We also discuss special cases to shed some light on the factors influencing the suboptimality bound
%We further refine the suboptimality bounds by considering special cases.
%Under mild conditions, we provide computable sub-optimality guarantees.
%, and we present special cases in which  these bounds can be further refined.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Performance bounds: depending on the submodularity ratio
% - Algorithm 2 is the first scalable algorithm with provable suboptimality guarantees for the minimization of a (possibly) approxi- mately supermodular function
% - Algorithm 4 is the first scalable algorithm with provable suboptimality guarantees for the minimum heterogeneous-cost set-selection subject to a constraint on an approximately supermodular function
% provide a computable lower bound for the submodularity ratio, and establish control-theoretic conditions for the validity of this lower bound.

In proving these results, we extend the literature 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% numerical experiments
In this paper we also motivate the importance of the \LQG control and sensing co-design problem, and demonstrate the effectiveness of the proposed algorithms in numerical experiments, by considering  
two application scenarios, namely, a 
\emph{sensing-constrained formation control} scenario and a 
\emph{resource-constrained robot navigation} scenario.   In particular, we present a Monte Carlo analysis for both scenarios, which demonstrates that 
(i) the proposed sensor selection strategy is near-optimal, and in particular, the resulting \LQG-cost 
(tracking performance) matches the optimal selection in all tested instances 
for which the optimal selection could be computed via a brute-force approach;
(ii) a more naive selection which attempts to minimize the state estimation covariance~\cite{jawaid2015submodularity}
(rather than the \LQG cost) has degraded \LQG tracking performance, often comparable to a random selection;
(iii) in the considered instances, the selection of a small subset of sensors per the proposed algorithms herein can ensure an \LQG cost that is 
close to the one obtained by using all available sensors, hence providing an effective alternative for control under 
sensing constraints~\cite{carlone2017attention}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\myparagraph{Comparison with the preliminary results in~\cite{Tzoumas18acc-scLGQG}} 
This paper extends the preliminary results presented in~\cite{Tzoumas18acc-scLGQG}.
%, and develops novel approximation algorithms for the optimization of an approximately supermodular set function. % in multiple directions. 
In~particular, the present paper provides a more comprehensive 
presentation of the \LQG control and sensing co-design problem, including both  
\emph{sensing-constrained \LQG control} (introduced in~\cite{Tzoumas18acc-scLGQG}) and the \emph{minimum-sensing \LQG control} problem (not previously published). Moreover, we generalize the original setup in~\cite{Tzoumas18acc-scLGQG} to account for heterogeneous sensor costs 
(in~\cite{Tzoumas18acc-scLGQG} each sensor has unit cost). 
Most of the technical results, including  Theorems~\ref{th:LQG_closed}--\ref{th:performance_LQGconstr}, Proposition~\ref{rem:extension}, as well as, Algorithms~\ref{alg:greedy_nonUniformCosts}--\ref{algLQGconstr:greedy_nonUniformCosts}
are novel, and have not been previously published. 
% For example, Algorithm~\ref{alg:greedy_nonUniformCosts} is the first scalable algorithm with provable suboptimality guarantees for the minimization of approximately supermodular functions subject to heterogeneous-cost set-selection constraints ---details on the novelty of Algorithms~\ref{alg:greedy_nonUniformCosts}--\ref{algLQGconstr:greedy_nonUniformCosts} are found in Section~\ref{sec:performanceGuarantees} (Remark~\ref{rem:novel1}) and Section~\ref{sec:performanceGuaranteesLQGconstr} (Remark~\ref{rem:novel2}).

%The rest of the paper is organized as follows.  
\myparagraph{Organization of the rest of the paper} In Section~\ref{sec:problemStatement} we formulate the  \LQG control and sensing co-design problems considered in this paper.
%, namely, the \emph{sensing-constrained \LQG control} problem and the \emph{minimum-sensing \LQG control} problem.  
In Section~\ref{sec:codesign} we provide scalable, near-optimal algorithms for these problems, and in Section~\ref{sec:guarantees} we characterize those algorithms' running time and approximation performance.  In Section~\ref{sec:exp} we present two practical applications of the co-design problems.
%, namely,
%\emph{sensing-constrained formation control} and 
%\emph{resource-constrained robot navigation}.
Section~\ref{sec:con} concludes the paper.  All proofs are found in the Appendix.  
%Below we introduce some notation.
\medskip

\myParagraph{Notation} 
Lowercase letters denote vectors and scalars (e.g., $v$), and uppercase letters denote matrices (e.g., $M$). We use calligraphic fonts to denote sets (e.g., $\calS$).
% Sets are denoted by sans script fonts e.g. $\setA$, $\setB$.  
% Non-bold face letters are used for scalars and indices (e.g. $j$) and function names (e.g. $f(\cdot)$). 
% The symbol $|\setA|$ denotes the cardinality of the set $\setA$.
The identity matrix of size~$n$ is denoted with~$\eye_n$ (the dimension index is omitted when it is clear from the context). 
% An $m \times n$ zero matrix is denoted by $\zero_{m\times n}$. 
% % The transpose of a vector or a matrix is represented by $\tran$, e.g. $\MX\tran$.
%The symbol $\|\cdot\|$ denotes the Euclidean norm for vectors and the spectral norm for matrices.
For a matrix $M$ and a vector $v$ of appropriate dimension, we define $\|v\|_M^2 \triangleq v\tran M v$.  For matrices $M_1,M_2,\ldots,M_k$, we let $\diag{M_1,M_2,\ldots,M_k}$ be the block diagonal matrix
with diagonal blocks $M_1,M_2,\ldots,M_k$.
% $M_1,M_2,\ldots,M_k$, $\diag{M_1,M_2,\ldots,M_k}$
% We let $\eye$ to be the identity matrix; for any matrices $M_1,M_2,\ldots,M_k$, $\diag{M_1,M_2,\ldots,M_k}$ to be the block diagonal matrix with diagonal elements the matrices $M_1,M_2,\ldots,M_k$; and
% for any matrix $M$, and vector $v$ of appropriate dimension, $\|v\|_M^2$ to be $v\tran M v$.



==> tex/JointControlSensingDesign.tex <==
%!TEX root = ../main.tex

\section{Joint Sensing and Control Design}

In this section we first present a separation principle that decouples sensing, estimation, and control, 
and allows designing them in cascade (Section~\ref{sec:separability}).
We then present a scalable algorithm for sensing and control design (Section~\ref{sec:designAlgorithm}).  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Separability of Optimal Sensing and Control Design}\label{sec:separability}

We characterize the jointly optimal control and sensing solutions to Problem~\ref{prob:LQG}, and prove that  
they can be found in two separate steps, where first the sensing design is computed, and second the {corresponding optimal control design is found.}

\begin{mytheorem}[Separability of optimal sensing and control design]\label{th:LQG_closed}
Let the sensor set $\calS^\star$ and the controllers $u_1^\star, u_2^\star, \ldots, u_T^\star$ be a solution to the sensing-constrained \LQG Problem~\ref{prob:LQG}. Then, $\calS^\star$  and $u_1^\star,$ $u_2^\star,\ldots,u_T^\star$ can be computed in cascade as follows: 
\begin{align}
\calS^\star &\in \argmin_{\calS \subseteq \calV, |\calS|\leq k}\sum_{t=1}^T\text{tr}[\Theta_t\Sigma\att{t}{t}(\calS)],\label{eq:opt_sensors}\\
u_t^\star&=K_t\hat{x}_{t,\calS^\star}, \quad t=1,\ldots,T\label{eq:opt_control}
\end{align}
where $\hat{x}\of{t}{\calS}$ is the Kalman estimator of the state $x_t$, i.e.,
$\hat{x}\of{t}{\calS}\triangleq\mathbb{E}(x_t|y\of{1}{\calS},y\of{2}{\calS},\ldots,y\of{t}{\calS})$,
and $\Sigma\att{t}{t}(\calS)$ is $\hat{x}\of{t}{\calS}$'s error covariance, i.e.,
$\Sigma\att{t}{t}(\calS)\triangleq\mathbb{E}[(\hat{x}\of{t}{\calS}-x_t)(\hat{x}\of{t}{\calS}-x_t)\tran]$~\cite[Appendix~E]{bertsekas2005dynamic}.
In~addition, the matrices $\Theta_t$ and $K_t$ are independent of the selected sensor set $\calS$, and  they are computed as follows: the matrices $\Theta_t$ and $K_t$ are the solution of the backward Riccati recursion
\beal\label{eq:control_riccati}
S_t &= Q_t + N_{t+1}, \\
N_t &= A_t\tran (S_t\inv+B_tR_t\inv B_t\tran)\inv A_t, \\
%\quad\mbox{ } = A_t\tran (S_t - S_t B_t M_t\inv B_t\tran S_t) A_t\\
%\quad\mbox{ } =A_t\tran S_t A_t-\Theta_t\\ 
M_t &= B_t\tran S_t B_t + R_t, \\ 
K_t &= - M_t\inv B_t\tran S_t A_t, \\ 
\Theta_t &= K_t\tran M_t K_t,
\eeal
with boundary condition $N_{T+1}=0$.
\end{mytheorem}

\begin{myremark}[Certainty equivalence principle]
The control gain matrices 
$K_1, K_2, \ldots, K_T$
are the same as the ones that make the controllers $(K_1x_1$, $K_1x_2,\ldots, K_T x_T)$ optimal for the perfect state-information version of Problem~\ref{prob:LQG}, where the state $x_t$ is known to the controllers~\cite[Chapter~4]{bertsekas2005dynamic}.
\end{myremark}

\input{tex/algorithm1}

Theorem~\ref{th:LQG_closed} decouples the design of the sensing from the controller design.
% implies that the optimal sensing and control design can be found in two steps, where in the first step an optimal sensing design is computed, and in the second step the corresponding optimal control design is found.  
Moreover, it suggests that once an optimal sensor set~$\calS^\star$ is found, then the optimal controllers are equal to $K_t\hat{x}\of{t}{\calS}$, which correspond to the standard \LQG control policy. 
This should not come as a surprise, since for a given sensing strategy, Problem~\ref{prob:LQG}
%the proposed sensing-constrained \LQG control problem 
reduces to standard \LQG control.

We conclude this section with a remark providing a more intuitive interpretation of the sensor design step in eq.~\eqref{eq:opt_sensors}.

%[Control theoretic interpretation of the sensor design cost~\eqref{eq:opt_sensors}]
\begin{myremark}[Control-aware sensor design]\label{rmk:interpretation}
In order to provide more insight on the cost function in~\eqref{eq:opt_sensors}, we rewrite it~as: 
\begin{align}
\!\!\!
\displaystyle\sum_{t=1}^{T}\text{tr}[\Theta_t\Sigma\att{t}{t}(\calS)] &\!=\!
\displaystyle\sum_{t=1}^{T}\mathbb{E}\left(\text{tr}\{[x_t-\hat{x}\of{t}{\calS}]\tran\Theta_t[x_t-\hat{x}\of{t}{\calS}]\}\right) \nonumber \\
%&\sum_{t=1}^{T}\mathbb{E}\left\{\text{tr}[(K_t x_t-K_t \hat{x}\of{t}{\calS})\tran M_t (K_t x_t-K_t \hat{x}\of{t}{\calS})]\right\},\\
&\!=\!
\displaystyle\sum_{t=1}^{T}\mathbb{E}\left( \| K_t x_t-K_t \hat{x}\of{t}{\calS}\|^2_{M_t} \right), \label{eq:interpretationRemark}
\end{align}
where in the first line we used the fact that 
$\Sigma\att{t}{t}(\calS) = \mathbb{E}\left[(x_t-\hat{x}\of{t}{\calS})(x_t-\hat{x}\of{t}{\calS})\tran\right]$, 
and in the second line we substituted the definition of $\Theta_t = K_t\tran M_t K_t$ from eq.~\eqref{eq:control_riccati}.

From eq.~\eqref{eq:interpretationRemark}, it is clear that each term 
$\text{tr}[\Theta_t\Sigma\att{t}{t}(\calS)]$ captures the expected control mismatch between the 
imperfect state-information controller $u\of{t}{\calS}=K_t\hat{x}\of{t}{\calS}$ (which is only aware of the 
measurements from the active sensors) and the  perfect state-information controller~$K_tx_t$.
%therefore the sensor selection attempts to minimize this mismatch.
This is an important distinction from the existing sensor selection literature. 
%e.g.,~\cite{jawaid2015submodularity}.
In particular, while standard sensor selection attempts to minimize the estimation covariance, for instance by 
minimizing
\begin{equation}
\sum_{t=1}^{T}\text{tr}[\Sigma\att{t}{t}(\calS)] \triangleq
\displaystyle\sum_{t=1}^{T}\mathbb{E}\left(\| x_t-\hat{x}\of{t}{\calS}\|^2_2 \right),\label{eq:interpretationRemark_kalman}
\end{equation}
the proposed \LQG cost formulation attempts to minimize the estimation error of only the informative states to the perfect state-information controller: for example, the contribution of all $x_t-\hat{x}\of{t}{\calS}$ in the null space of $K_t$ to the total control mismatch in eq.~\eqref{eq:interpretationRemark} is zero.
% For instance, depending on the \LQG weight matrices $Q_t$ and $R_t$ 
% the matrix $K_t$ may have a null space corresponding to states that are irrelevant 
% for the sake of control, and since the null space of $K_t$ dictates the null space of $\Theta_t$, 
% this fact will be captured by~\eqref{eq:opt_sensors}.
Hence,  in contrast to minimizing the cost function in eq.~\eqref{eq:interpretationRemark_kalman}, minimizing the cost function in eq.~\eqref{eq:interpretationRemark} results to a control-aware sensing~design.
 
%only attempt to 
% the mean square estimation error that disturbs the controller 
%  away from the perfect state-information controller~$K_tx_t$.
% %the reason for the latter is twofold:
% \begin{itemize}
% \item each matrix $\Theta_t$
% %, computed in Algorithm~\ref{alg:greedy}'s lines 6--9, 
% incorporates how the Kalman estimation error $x_t-\hat{x}\of{t}{\calS}$ perturbs the control policy $u\of{t}{\calS}=K_t\hat{x}\of{t}{\calS}$ away from the perfect state-information control policy $K_t x_t$, since (i)~$u\of{t}{\calS}=K_t\hat{x}\of{t}{\calS}=K_tx_t-K_t(x_t-\hat{x}\of{t}{\calS})$; and (ii)~the matrices $\Theta_t$ and $K_t$ have the same null space, since $\Theta_t= K_t\tran M_t K_t$ per Algorithm~\ref{alg:greedy}'s line~8.  
% \item For any sensor set $\calS\subseteq \calV$, 
% i.e., each $\text{tr}[\Theta_t\Sigma\att{t}{t}(\calS)]$ captures the mean square error that disturbs the controller $u_{t,\calS}=K_t\hat{x}\of{t}{\calS}$ away from the perfect state-information controller~$K_tx_t$.
% \end{itemize}
\end{myremark}


% Notwithstanding, since the optimization problem in eq.~\eqref{eq:opt_sensors} can be intractable, being a combinatorial problem, the following question arises:  If only an approximate solution $\algS$ can be found for the optimization problem in eq.~\eqref{eq:opt_sensors}, are the corresponding controllers $K_t \hat{x}_{t,\algS}$ for all $t=1,2,\ldots,T$ still optimal for Problem~\ref{prob:LQG}?  We~answer affirmatively this question, \mbox{with the following theorem.}
% \begin{mytheorem}[Separation of sensing and control policy design]\label{th:separation}
% Given any selected sensor set $\calS\subset \calV$ in Problem~\ref{prob:LQG}, the controllers  $(K_1\hat{x}_{1,\calS},$ $K_2\hat{x}_{2,\calS},\ldots,K_T\hat{x}_{T,\calS})$ are optimal for Problem~\ref{prob:LQG}, since for the value of Problem~\ref{prob:LQG} it holds
% \begin{align*}
% &\hspace{-1.1em}\min_{\scriptsize \begin{array}{c}
% \calS \subseteq \calV, |\calS|\leq k,\\
% u_{t,\calS}\in \mathbb{R}^{m_t}
% \end{array}} \sum_{t=1}^{T}\mathbb{E}\left(\|x\at{t+1}\|^2_{Q_t}+\|u_{t,\calS}\|^2_{R_t}\right)=\\
% &\min_{\calS \subseteq \calV, |\calS|\leq k} \sum_{t=1}^{T}\mathbb{E}\left(\|x\at{t+1}\|^2_{Q_t}+\|K_t \hat{x}_{t,\calS}\|^2_{R_t}\right).
% \end{align*}
% \end{mytheorem}

\input{tex/algorithm2}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Scalable Near-optimal Sensing and Control Design}\label{sec:designAlgorithm}

This section proposes a practical design algorithm for Problem~\ref{prob:LQG}.
The pseudo-code of the algorithm is presented in Algorithm~\ref{alg:overall}.
Algorithm~\ref{alg:overall} follows the result of Theorem~\ref{th:LQG_closed}, 
and jointly designs sensing and control by first 
%which proves that the jointly optimal design can be obtained by first 
computing an active sensor set (line 1 in Algorithm~\ref{alg:overall}) and then computing the control policy
(line 2 in Algorithm~\ref{alg:overall}).
We discuss each step of the design process in the rest of this section.
%, the algorithm 
%first computes the optimal sensor set (by calling Algorithm~\ref{alg:greedy}), and then computes an
%optimal control policy,
% simply 
% calls two subroutines, Algorithm~\ref{alg:greedy} and Algorithm~\ref{alg:control}, which design the sensing and the control policy, respectively.
% The two algorithms are described in the following, while the corresponding performance guarantees are given in Section~\ref{sec:guarantees}.
% implies that the sensing-constrained \LQG Problem~\ref{prob:LQG} can be solved using an algorithm of the form of Algorithm~\ref{alg:overall}.  In particular, Algorithm~\ref{alg:overall} constructs a solution~$(\algS,$  $ u_{1,\algS},u_{2,\algS}, \ldots,u_{T,\algS})$ for Problem~\ref{prob:LQG}, where $\algS$ is the sensor set, and $(u_{1,\algS}, u_{2,\algS}, \ldots,$ $u_{T,\algS})$ are the controllers, in two steps:

%\setcounter{paragraph}{0}
\subsubsection{Near-optimal Sensing design}
The optimal sensor design can be computed by solving the optimization problem in eq.~\eqref{eq:opt_sensors}.
%Algorithm~\ref{alg:greedy} attempts to design a sensing policy by solving the optimization problem~\eqref{eq:opt_sensors}.
The problem is combinatorial in nature, since it requires to select a subset of elements of cardinality $k$ out of all the available sensors that 
induces the smallest cost. %Moreover, 
%the dependency of $\Sigma\att{t}{t}(\calS)$ (and hence the cost) on the set $\calS$ 
%if highly nonlinear, which implies that one cannot 

In this section we propose a greedy algorithm, whose pseudo-code is given in Algorithm~\ref{alg:greedy}, 
that computes a (possibly approximate) solution to the problem in eq.~\eqref{eq:opt_sensors}. 
Our interest towards this greedy algorithm is motivated by the fact that it is scalable 
(in Section~\ref{sec:guarantees} we show that its complexity is linear in the number of available sensors) 
and is provably close to the optimal solution of the problem in eq.~\eqref{eq:opt_sensors} 
\mbox{(we provide suboptimality bounds in Section~\ref{sec:guarantees}).}


Algorithm~\ref{alg:greedy} computes the matrices $\Theta_t$ ($\allT$)
which appear in the cost function in eq.~\eqref{eq:opt_sensors} (line~\ref{line:computeThetas}). Note that these matrices are independent 
on the choice of sensors. 
The~set of active sensors $\algS$ is initialized to the empty set (line~\ref{line:initialize}). 
The~``while loop'' in line~\ref{line:while} will be executed~$k$ times and at each time 
a sensor is greedily added to the set of active sensors~$\algS$. 
In~particular, the ``for loop'' in lines~\ref{line:startFor1}-\ref{line:endFor1} 
 computes the estimation covariance resulting by adding a sensor to the current 
active sensor set and the corresponding cost (line~\ref{line:cost}). 
Finally, the sensor inducing the smallest cost is selected (line~\ref{line:best_a}) 
and added \mbox{to the current set of active sensors (line~\ref{line:add_a}).}
%Then, line~\ref{line:best_a} computes the~\eqref{eq:opt_sensors} resulting  
%selects greedily a sensor set~$\algS$ to minimize (possibly approximately) the set function $\sum_{t=1}^{T}\text{tr}[\Theta_t\Sigma\att{t}{t}(\calS)]$. 

% Overall, Algorithm~\ref{alg:greedy} greedily selects  a sensor set $\algS$ in the attempt to minimize the cost in eq.~\eqref{eq:opt_sensors};
% as per Remark~\ref{rmk:interpretation}, this  
% bring the imperfect state-information controllers $u\of{t}{\calS}$ close to the perfect state-information optimal controllers $K_t x_t$ (Remark~\ref{rmk:interpretation}), and as a result, to achieve the minimum value for Problem~\ref{prob:LQG}.

%\input{tex/algorithm3}

\subsubsection{Control policy design}
The optimal control design is computed as in eq.~\eqref{eq:opt_control}, where
%The controller design is identical to what prescribed by standard \LQG theory.
the control policy matrices \mbox{$K_1,K_2,\ldots,K_T$ are obtained 
from the recursion~in~eq.~\eqref{eq:control_riccati}.}
 

% For the sake of completeness, we recall the involved computation in Algorithm~\ref{alg:control}.
% {eq:control_riccati}
% In line~2, Algorithm~\ref{alg:overall} computes the control matrices $K_1,K_2,\ldots,K_T$, using Algorithm~\ref{alg:control}.  
% Then, Theorem~\ref{th:separation} implies that for the selected sensor set~$\algS$ in line~1, and for any measurements $y_{1,\algS},y_{2,\algS},\ldots,y_{t,\algS}$ up to time~$t$,  the optimal controller 
% $u_t$ is $K_t\hat{x}_{t,\algS}$.
%For completeness we mention Algorithm 2 (one of the subroutines called in Alg 1), and for convenience we have alg 2 output M and K

In the following section we characterize the approximation and running-time performance of Algorithm~\ref{alg:overall}.

==> tex/ProblemFormulation.tex <==
%!TEX root = ../main.tex

\section{Sensing-Constrained LQG Control} 
\label{sec:problemStatement}

In this section we formalize the sensing-constrained LQG control problem considered in this paper. 
We start by introducing the notions of  \emph{system},  \emph{sensors}, and  \emph{control policies}.
%To this end, we start with the systems, sensors, and control policies considered in this paper.  In more detail:
\paragraph{System} We consider a standard discrete-time (possibly time-varying) 
linear system with additive Gaussian noise:  
%In~more~detail, if we let $T$ to denote a finite time-horizon, we consider systems of the form
\begin{equation}
x\at{t+1}=A_tx_t+B_tu_t + w_t, \quad t = 1, 2, \ldots, T,\label{eq:system}
\end{equation}
where $x_t \in \mathbb{R}^{n_t}$ represents the state of the system at time~$t$, $u_t \in \mathbb{R}^{m_t}$ represents the control action, $w_t$ represents the process noise, and 
$T$ is a finite time horizon. In~addition, we~consider the system's initial condition $x_1$ to be a Gaussian random variable with covariance~$\Sigma\att{1}{0}$, and $w_t$ to be a Gaussian random variable with mean zero and covariance $W_t$, such that $w_t$ is independent of $x_1$ and $w_{t'}$ for all $t'=1,2,\ldots,T$, $t'\neq t$.

\paragraph{Sensors} We consider the case where we have a (potentially large) set of available sensors, which take noisy linear observations of the system's state. %, corrupted with additive Gaussian noise.  
In particular, let~$\calV$  be a set of indices such that each index $i\in\calV$ uniquely identifies a 
sensor that can be used to observe the state of the system. We consider sensors of the form
\begin{equation}
y_{i,t}=C_{i,t}x_t+v_{i,t}, \quad i \in \calV,\label{eq:sensors}
\end{equation}
where $y_{i,t}\in \mathbb{R}^{p_{i,t}}$ represents the measurement of sensor $i$ at time~$t$, and $v_{i,t}$ represents the measurement noise of sensor~$i$.  We assume $v_{i,t}$ to be a Gaussian random variable with mean zero and positive definite covariance $V_{i,t}$, such that~$v_{i,t}$ is independent of $x_1$, and of $w_{t'}$ for any $t'\neq t$, and independent of $v_{i',t'}$ for all $t'\neq t$, and any $i'\in\calV$, $i' \neq i$.

In this paper we are interested in the case 
%As clarified in the statement of the sensing-constrained \LQG Problem~\ref{prob:LQG} below, we are interested in the case 
in which 
we cannot use all the available sensors, and as a result, we need to
select a convenient subset of sensors in $\calV$ to maximize our control performance 
(formalized in Problem~\ref{prob:LQG} below). 
%We can the set of selected sensors the \emph{active sensor set}.

\begin{mydef}[Active sensor set and measurement model]\label{notation:sensor_noise_matrices}
Given a set of available sensors $\calV$, we say that 
$\calS \subset \calV$ is an \emph{active sensor set} if we can observe 
the measurements from each sensor $i\in \calS$ for all $t = 1,2,\ldots, T$.
Given an active sensor set $\calS=\{i_1, i_2 \ldots, i_{|\calS|}\}$,
we define the following quantities % vector and matrices
\beal
y_{t}(\calS) & \triangleq& [y_{i_1,t}\tran, y_{i_2,t}\tran, \ldots, y_{i_{|\calS|},t}\tran]\tran,\\
C_t(\calS) & \triangleq& [C\at{i_1,t}\tran, C\at{i_2,t}\tran, \ldots, C\at{i_{|\calS|},t}\tran]\tran, \\
V_t(\calS)& \triangleq& \text{diag}[V\at{i_1,t}, V\at{i_2,t}, \ldots,V\at{i_{|\calS|},t}]
\eeal
% For any time $t=1,2,\ldots,T$, and any sensor set $\calS \subseteq \calV$, let $C_t(\calS)$ to be the measurement matrix corresponding to the selected sensors in $\calS$, i.e., for $\calS=\{i_1, i_2 \ldots, i_{|\calS|}\}$,
% $$C_t(\calS) = [C\at{i_1,t}\tran, C\at{i_2,t}\tran, \ldots, C\at{i_{|\calS|},t}\tran]\tran,$$
% and $V_t(\calS)$ to be the noise covariance matrix corresponding to the selected sensors in $\calS$, i.e., for $\calS=\{i_1, i_2 \ldots, i_{|\calS|}\}$,
% $$V_t(\calS)= \text{diag}[V\at{i_1,t}, V\at{i_2,t}, \ldots,V\at{i_{|\calS|},t}].$$
which lead to the definition of the \emph{measurement model}:
%active sensor set model:
\begin{equation}
y_{t}(\calS) = C_t(\calS) x_t + v_{t}(\calS)\label{eq:activeSensors}
\end{equation}
where $v_t(\calS)$ is a zero-mean Gaussian noise with covariance~$V_t(\calS)$.
Despite the availability of a possibly large set of sensors $\calV$, our observer 
will only have access to the measurements produced by the active sensors.
% In other words, despite having a large set of sensors $\calV$ we can only 
% We also
% and if we also let $y_{t,\calS}$ be the vector of all sensor measurements $y_{i,t}$ such that $i \in \calS$
% In~more~detail, if we let $\calS$ to be the active subset of available sensors in $\calV$ across all $t=1,2,\ldots,T$, that is, 
% \begin{itemize}
% \item $i\in \calS$ if sensor $i$ is active for all $t = 1,2,\ldots, T$,
% \item $i\notin \calS$ if sensor $i$ is inactive for all $t = 1,2,\ldots, T$,
% \end{itemize}
% and if we also let $y_{t,\calS}$ be the vector of all sensor measurements $y_{i,t}$ such that $i \in \calS$
\end{mydef}


The following paragraph formalizes how 
%Before presenting Problem~\ref{prob:LQG}, we remark how 
the choice of the active sensors affects the control policies.
%The indices in $\calV$ can be understood as unique identifiers 
%of the available sensors.

\paragraph{Control policies}  We consider control policies~$u_t$ for all $t=1,2,\ldots,T$ 
that are only informed by the measurements collected by the active sensors:
% whose available information is composed from all the collected measurements up to time $t$ from the selected subset of sensors in $\calV$ to be active across all $t=1,2,\ldots,T$.  , we consider control policies of the form
\begin{equation*}
u_t = u\of{t}{\calS}= u_t(y\of{1}{\calS}, y\of{2}{\calS}, \ldots, y\of{t}{\calS}), \quad t = 1,2,\ldots,T.
\end{equation*}
Such policies are called \emph{admissible}.  

In this paper, we want to find a small set of active sensors $\calS$, 
%to be the active subset of available sensors in $\calV$ across all $t=1,2,\ldots, T$, 
and admissible controllers $u\of{1}{\calS}, u\of{2}{\calS},\ldots, u\of{T}{\calS}$, to solve the following sensing-constrained \LQG control problem.

\begin{myproblem}[Sensing-constrained LQG control]\label{prob:LQG}
Find a sensor set $\calS \subset \calV$ of cardinality at most $k$ to be active across all times $t=1,2,\ldots, T$, and control policies $u\of{1:T}{\calS} \triangleq \{u\of{1}{\calS},$ $u\of{2}{\calS}, \ldots, u\of{T}{\calS}\}$, that minimize the \LQG cost function:
\begin{equation}
\label{eq:sensingConstrainedLQG}
\min_{\scriptsize \begin{array}{c}
\calS \subseteq \calV, |\calS|\leq k,\\
u\of{1:T}{\calS} % \in \mathbb{R}^{m_t}
\end{array}} \sum_{t=1}^{T}\mathbb{E}\left[\|x\of{t+1}{\calS}\|^2_{Q_t} +\|u\of{t}{\calS}\|^2_{R_t}\right],
\end{equation}
where the state-cost matrices $Q_1, Q_2, \ldots, Q_T$ are positive semi-definite, the control-cost matrices $R_1, R_2, \ldots, R_T$ are positive definite, 
 % $ \sum_{t=1}^{T}\mathbb{E}\left[\|x\at{t+1}\|^2_{Q_t} +\|u_{t,\calS}\|^2_{R_t}\right]$ is minimized, where ; formally, solve the optimization problem
and the expectation is taken with respect to the initial condition $x_1$, the process noises $w_1, w_2, \ldots, w_T$, and the measurement noises $v\of{1}{\calS}, v\of{2}{\calS}, \ldots, v\of{T}{\calS}$.
%, where $v_{t,\calS}$ is the vector of all measurement noises $v_{i,t}$ such that $i \in \calS$.
\end{myproblem}

Problem~\ref{prob:LQG} generalizes the imperfect state-information \LQG control problem from the case where all sensors in $\calV$ are active, and only optimal control policies are to be found~\cite[Chapter~5]{bertsekas2005dynamic}, to the case where only a few sensors in $\calV$ can be active, and both optimal sensors and control policies are to be found jointly. 
While we already noticed that admissible control policies depend on the active sensor set $\calS$, it is worth noticing that 
this in turn implies that the state evolution also depends on $\calS$; for this reason we write $x\of{t+1}{\calS}$ in eq.~\eqref{eq:sensingConstrainedLQG}.
The intertwining between control and sensing calls for a joint design strategy.
% Since the choice of the control action and the ac
% In~more~detail, in Problem~\ref{prob:LQG} the optimal sensors and control policies are to be found in tandem, since for different active sensor sets~$\calS$, the available information $(y_{1,\calS}, y_{2,\calS}, \ldots, y_{t,\calS})$ to each admissible control policy~$u_{t,\calS}$ changes.  
In~the following section we focus on the design of a jointly optimal control {and sensing solution to Problem~\ref{prob:LQG}.}

% \setcounter{mynotation}{1}
% \begin{mynotation}\label{notation:sensor_noise_matrices}
% For any time $t=1,2,\ldots,T$, and any sensor set $\calS \subseteq \calV$, let $C_t(\calS)$ to be the measurement matrix corresponding to the selected sensors in $\calS$, i.e., for $\calS=\{i_1, i_2 \ldots, i_{|\calS|}\}$,
% $$C_t(\calS) = [C\at{i_1,t}\tran, C\at{i_2,t}\tran, \ldots, C\at{i_{|\calS|},t}\tran]\tran,$$
% and $V_t(\calS)$ to be the noise covariance matrix corresponding to the selected sensors in $\calS$, i.e., for $\calS=\{i_1, i_2 \ldots, i_{|\calS|}\}$,
% $$V_t(\calS)= \text{diag}[V\at{i_1,t}, V\at{i_2,t}, \ldots,V\at{i_{|\calS|},t}].$$
% \end{mynotation}

==> tex/algorithm1.tex <==
%!TEX root = ../main.tex

\begin{algorithm}[t]
\caption{\mbox{Joint Sensing and Control design \hspace{-.25mm}for \hspace{-.25mm}Problem~\ref{prob:LQG}.}}
\begin{algorithmic}[1]
\REQUIRE  Time horizon $T$, available sensor set $\calV$, covariance matrix $\initialCovariance$ of initial condition $x_1$; for all $t=1,2,\ldots, T$, system matrix $A_t$, input matrix $B_t$, LQG cost matrices $Q_t$ and $R_t$, process noise covariance matrix $W_t$; and for all sensors $i \in \calV$, measurement matrix $C_{i,t}$, and measurement noise covariance matrix~$V_{i,t}$.
\ENSURE Active sensors $\widehat{\mathcal{S}}$, and control matrices $K_1, \ldots, K_T$.
\STATE{$\widehat{\calS}$ is returned by Algorithm~\ref{alg:greedy} that finds a (possibly approximate) solution to the optimization problem in eq.~\eqref{eq:opt_sensors};
% (Algorithm~\ref{alg:greedy} in Section~\ref{sec:greedy});
 }
\STATE{$K_1,\ldots,K_T$ are computed using the recursion in eq.~\eqref{eq:control_riccati}.
% (Algorithm~\ref{alg:control} in current section);
 }
\end{algorithmic} \label{alg:overall}
\end{algorithm}

==> tex/algorithm2.tex <==
%!TEX root = ../main.tex

\begin{algorithm}[t]
\caption{Sensing design for Problem~\ref{prob:LQG}.}
\begin{algorithmic}[1]
\REQUIRE Time horizon $T$, available sensor set $\calV$, covariance matrix $\initialCovariance$ of system's initial condition $x_1$, and for any time $t =1,2,\ldots, T$, any sensor $i \in \calV$, process noise covariance matrix $W_t$, measurement matrix $C_{i,t}$, and measurement noise covariance matrix $V_{i,t}$.
\ENSURE Sensor set $\algS$.
\STATE Compute $\Theta_1,\Theta_2,\ldots,\Theta_T$ using recursion in eq.~\eqref{eq:control_riccati}; \label{line:computeThetas}
%are returned by Algorithm~\ref{alg:control};
\STATE $\algS\leftarrow\emptyset$; \quad $i \leftarrow 0$; \label{line:initialize}
\WHILE {$i < k$}   \label{line:while}
	\FORALL {$a\in \calV\setminus\algS$} \label{line:startFor1}
	\STATE{$\algS_a\leftarrow \algS\cup \{a\}$; \quad $\initialCovariance(\algS_a)\leftarrow \initialCovariance$;}
	\FORALL {$t = 1,\ldots, T$}
	\vspace{0.3mm}
	\STATE{$\Sigma\att{t}{t}(\algS_a)\leftarrow$}
	\STATE{$[ 
	\Sigma\att{t}{t-1}(\algS_a)\inv + C_t(\algS_a)\tran V_t(\algS_a)\inv C_t(\algS_a)]\inv$;} 
	\STATE{$\Sigma\att{t+1}{t}(\algS_a)\leftarrow A_{t} \Sigma\att{t}{t}(\algS_a) A_{t}\tran + W_{t}$;}
	\ENDFOR
	\STATE{$\text{cost}_a \leftarrow \sum_{t=1}^T\text{tr}[\Theta_t\Sigma\att{t}{t}(\algS_a)]$;} \label{line:cost}
	\ENDFOR \label{line:endFor1}
\STATE{$a_i \leftarrow \arg\min_{a \in \calV\setminus \mathcal{S}} \text{cost}_a$;} \label{line:best_a}
\STATE{$\algS\leftarrow \algS \cup \{a_i\}$; \quad $i \leftarrow i+1$;} \label{line:add_a}
\ENDWHILE
\end{algorithmic} \label{alg:greedy}
\end{algorithm}

==> tex/figure_formation_costVShorizon.tex <==
%!TEX root = ../main.tex

\renewcommand{\mpw}{4.5cm}
\begin{figure}[t]
\hspace{-4mm}
\begin{minipage}{\textwidth}
\begin{tabular}{cc}%
\begin{minipage}{\mpw}%
\centering
\includegraphics[width=1.05\columnwidth]{code/results-formationControl-costOverHorizon/figure-formationControl-singleRun-T20-maxT20-maxT20-het0-mpc0-n4-k6} \\
(a) homogeneous 
\end{minipage}
& 
\begin{minipage}{\mpw}%
\centering%
\includegraphics[width=1.05\columnwidth]{code/results-formationControl-costOverHorizon/figure-formationControl-singleRun-T20-maxT20-maxT20-het1-mpc0-n4-k6} \\
(b) heterogeneous 
\end{minipage}
\end{tabular}
\end{minipage}%
\vspace{-1mm}
\caption{\label{fig:snapshots}
Snapshots of the feature selection performed by the different techniques  during a sharp
}\vspace{-5mm}
\end{figure}
